Physical Processes in the Interstellar Medium

Interstellar space is filled with a dilute mixture of charged particles, atoms, molecules and dust grains, called the interstellar medium (ISM). Understanding its physical properties and dynamical behavior is of pivotal importance to many areas of astronomy and astrophysics. Galaxy formation and evolution, the formation of stars, cosmic nucleosynthesis, the origin of large complex, prebiotic molecules and the abundance, structure and growth of dust grains which constitute the fundamental building blocks of planets, all these processes are intimately coupled to the physics of the interstellar medium. However, despite its importance, its structure and evolution is still not fully understood. Observations reveal that the interstellar medium is highly turbulent, consists of different chemical phases, and is characterized by complex structure on all resolvable spatial and temporal scales. Our current numerical and theoretical models describe it as a strongly coupled system that is far from equilibrium and where the different components are intricately linked together by complex feedback loops. Describing the interstellar medium is truly a multi-scale and multi-physics problem. In these lecture notes we introduce the microphysics necessary to better understand the interstellar medium. We review the relations between large-scale and small-scale dynamics, we consider turbulence as one of the key drivers of galactic evolution, and we review the physical processes that lead to the formation of dense molecular clouds and that govern stellar birth in their interior.

==> Readme <==
Title: Physical Processes in the Interstellar Medium

Authors: Ralf S. Klessen, Simon C. O. Glover (Universit\"at Heidelberg, Zentrum
 f\"ur Astronomie, Institut f\"ur Theoretische Astrophysik)

Categories: astro-ph.GA

Comments: Lecture notes given at the 43rd Saas Fee Advanced School, March
 11-16, 2013, Villars-sur-Ollon, Switzerland -- 191 pages, 23 figures.
 Links to the video recording of the lectures :
 http://lastro.epfl.ch/conferences/sf2013/videos2.cgi



\\
 Interstellar space is filled with a dilute mixture of charged particles,
atoms, molecules and dust grains, called the interstellar medium (ISM).
Understanding its physical properties and dynamical behavior is of pivotal
importance to many areas of astronomy and astrophysics. Galaxy formation and
evolution, the formation of stars, cosmic nucleosynthesis, the origin of large
complex, prebiotic molecules and the abundance, structure and growth of dust
grains which constitute the fundamental building blocks of planets, all these
processes are intimately coupled to the physics of the interstellar medium.
However, despite its importance, its structure and evolution is still not fully
understood. Observations reveal that the interstellar medium is highly
turbulent, consists of different chemical phases, and is characterized by
complex structure on all resolvable spatial and temporal scales. Our current
numerical and theoretical models describe it as a strongly coupled system that
is far from equilibrium and where the different components are intricately
linked together by complex feedback loops. Describing the interstellar medium
is truly a multi-scale and multi-physics problem. In these lecture notes we
introduce the microphysics necessary to better understand the interstellar
medium. We review the relations between large-scale and small-scale dynamics,
we consider turbulence as one of the key drivers of galactic evolution, and we
review the physical processes that lead to the formation of dense molecular
clouds and that govern stellar birth in their interior.
\\


------------------------------------------------------------------------------------


Title: Modeling Physical Processes at Galactic Scales and Above

Authors: Nickolay Y. Gnedin (Particle Astrophysics Center, Fermi National Accelerator Laboratory,
Kavli Institute for Cosmological Physics, The University of Chicago)

Categories: astro-ph.GA

Comments: Lecture notes given at the 43rd Saas Fee Advanced School, March
 11-16, 2013, Villars-sur-Ollon, Switzerland -- 87 pages, 54 figures.
 Links to the video recording of the lectures :
 http://lastro.epfl.ch/conferences/sf2013/videos3.cgi
\\
What should these lectures be? The subject assigned to us is so broad that many
books can be written about it. So, in planning these lectures I had several options.
One would be to focus on a narrow subset of topics and to cover them in great
detail. Such a subset necessarily would be highly personal and useful to a few read-
ers at best. Another option would be to give a very shallow overview of the whole
field, but then it won?t be very much different from a highly compressed version of
a university course (which anyone can take if they wish so).
So, I decided to be selfish and to prepare these lectures as if I was teaching my
own graduate student. Given my research interests, I selected what the student would
need to know to be able to discuss science with me and to work on joint research
projects. So, the story presented below is both personal and incomplete, but it does
cover several subjects that are poorly represented in the existing textbooks (if at all).
Some of topics I focus on below are closely connected, others are disjoint, some
are just side detours on specific technical questions. There is an overlapping theme,
however. Our goal is to follow the cosmic gas from large scales, low densities, (rel-
atively) simple physics to progressively smaller scales, higher densities, closer rela-
tion to galaxies, and more complex and uncertain physics. So, we (you - the reader,
and me - the author) are going to follow a "yellow brick road" from the gas well be-
yond any galaxy confines to the actual sites of star formation and stellar feedback.
On the way we will stop at some places for a tour and run without looking back
through some others. So, the road will be uneven, but I hope that some readers find
it useful.
\\



------------------------------------------------------------------------------------


Title: High performance computing and numerical modelling


Authors: Volker Springel (Heidelberg Institute for Theoretical Studies, Heidelberg University, Zentrum für Astronomie)

Categories: astro-ph.GA

Comments: Lecture notes given at the 43rd Saas Fee Advanced School, March
 11-16, 2013, Villars-sur-Ollon, Switzerland -- 108 pages, 36 figures.
 Links to the video recording of the lectures :
 http://lastro.epfl.ch/conferences/sf2013/videos1.cgi

\\
Numerical methods play an ever more important role in astrophysics. This is
especially true in theoretical works, but of course, even in purely
observational projects, data analysis without massive use of computational
methods has become unthinkable. The key utility of computer simulations comes
from their ability to solve complex systems of equations that are either
intractable with analytic techniques or only amenable to highly approximative
treatments. Simulations are best viewed as a powerful complement to analytic
reasoning, and as the method of choice to model systems that feature enormous
physical complexity such as star formation in evolving galaxies, the topic of
this 43rd Saas Fee Advanced Course. The organizers asked me to lecture about
high performance computing and numerical modelling in this winter school, and to
specifically cover the basics of numerically treating gravity and hydrodynamics
in the context of galaxy evolution. This is still a vast field, and I
necessarily had to select a subset of the relevant material. The written notes
presented here quite closely follow the lectures as held in Villars-sur-Ollon,
which were meant to provide a general overview about some of the most pertinent
techniques that may be relevant for students working on numerical models of
galaxy evolution and star formation. The discussion is hence often at an
introductory level, giving precedence to a presentation of the main numerical
concepts rather than to a mathematically detailed exposition of the techniques.
\\



